The Impact of Using Regression Models to Build Defect Classifiers

It is common practice to discretize continuous defect counts into defective and non-defective classes and use them as a target variable when building defect classifiers (discretized classifiers). However, this discretization of continuous defect counts leads to information loss that might affect the performance and interpretation of defect classifiers. Another possible approach to build defect classifiers is through the use of regression models then discretizing the predicted defect counts into defective and non-defective classes (regression-based classifiers). In this paper, we compare the performance and interpretation of defect classifiers that are built using both approaches (i.e., discretized classifiers and regression-based classifiers) across six commonly used machine learning classifiers (i.e., linear/logistic regression, random forest, KNN, SVM, CART, and neural networks) and 17 datasets. We find that: i) Random forest based classifiers outperform other classifiers (best AUC) for both classifier building approaches; ii) In contrast to common practice, building a defect classifier using discretized defect counts (i.e., discretized classifiers) does not always lead to better performance. Hence we suggest that future defect classification studies should consider building regression-based classifiers (in particular when the defective ratio of the modeled dataset is low). Moreover, we suggest that both approaches for building defect classifiers should be explored, so the best-performing classifier can be used when determining the most influential features.

==> RelatedWork.tex <==
\begin{thebibliography}{1}

\bibitem{1}
Tassey, Gregory. "The economic impacts of inadequate infrastructure for software testing." National Institute of Standards and Technology, RTI Project 7007.011 (2002).
\bibitem{2}
Andersson, Carina. "A replicated empirical study of a selection method for software reliability growth models." Empirical Software Engineering 12.2 (2007): 161-182.

\bibitem{3}
Arar, Ömer Faruk, and Kürşat Ayan. "Software defect prediction using cost-sensitive neural network." Applied Soft Computing 33 (2015): 263-277.
\bibitem{4}
Ceylan, Evren, F. Onur Kutlubay, and Ayse B. Bener. "Software defect identification using machine learning techniques." 32nd EUROMICRO Conference on Software Engineering and Advanced Applications (EUROMICRO'06). IEEE, 2006.

\bibitem{5}
Fagan, Michael E. "Design and code inspections to reduce errors in program development." Pioneers and Their Contributions to Software Engineering. Springer Berlin Heidelberg, 2001. 301-334.

\bibitem{6}
 R. Moser, W. Pedrycz, and G. Succi. A comparative analysis of the efficiency of change metrics and static code attributes for defect prediction. In Proceedings of the 30th International Conference on Software Engineering, pages 181–190. ACM, May 2008
 
\bibitem{7}
R. Mullen and S. Gokhale. Software Defect Rediscoveries: A Discrete Lognormal Model. In Proceedings of the 16th IEEE International Symposium on Software Reliability Engineering,
pages 203–212. IEEE, 2005.

\bibitem{8}
F. Shull, V. Basili, B. Boehm, A. Brown, P. Costa, M. Lindvall, D. Port, I. Rus, R. Tesoriero, and M. Zelkowitz. What we have learned about fighting defects. In Proceedings of the
8th IEEE Symposium on Software Metrics, pages 249–258, 2002.

\bibitem{9}
D'Ambros, Marco, Michele Lanza, and Romain Robbes. "An extensive comparison of bug prediction approaches." 2010 7th IEEE Working Conference on Mining Software Repositories (MSR 2010). IEEE, 2010.

\bibitem{10}
Kim, Sunghun, et al. "Predicting faults from cached history." Proceedings of the 29th international conference on Software Engineering. IEEE Computer Society, 2007.

\bibitem{11}
A. E. Hassan. Predicting Faults Using the Complexity of Code Changes. In Proceedings of the International Conference on Software Engineering (ICSE), pages 78–88, 2009.

\bibitem{12}

M. Cataldo, A. Mockus, J. Roberts, and J. Herbsleb. Software Dependencies, Work Dependencies, and Their Impact on Failures. IEEE Transactions on Software Engineering (TSE), 35(6):864–878, 2009.

\bibitem{13}

S. McIntosh, Y. Kamei, B. Adams, and A. E. Hassan. The Impact of Code Review Coverage and Code Review Participation on Software Quality. In Proceedings of the Working Conference on Mining Software Repositories (MSR), pages 192–201, 2014.

\bibitem{14}

A. Mockus. Organizational Volatility and its Effects on Software Defects. In Proceedings of the International Symposium on Foundations of Software Engineering (FSE), pages 117–127, 2010.


\bibitem{15}
Hall, Tracy, et al. ”A systematic literature review on fault prediction performance in software engineering.” IEEE Transactions on Software Engineering 38.6 (2012): 1276-1304.

\bibitem{16}

Cohen, Jacob. "The cost of dichotomization." (1983).

\bibitem{17}

Altman, Douglas G., and Patrick Royston. "The cost of dichotomising continuous variables." Bmj 332.7549 (2006): 1080.

\bibitem{18}
Royston, Patrick, Douglas G. Altman, and Willi Sauerbrei. "Dichotomizing continuous predictors in multiple regression: a bad idea." Statistics in medicine 25.1 (2006): 127-141.

\bibitem{19}
Austin, Peter C., and Lawrence J. Brunner. "Inflation of the type I error rate when a continuous confounding variable is categorized in logistic regression analyses." Statistics in medicine 23.7 (2004): 1159-1178.

\bibitem{20}
MacCallum, Robert C., et al. "On the practice of dichotomization of quantitative variables." Psychological methods 7.1 (2002): 19.

\bibitem{21}
Rohit Singh, Tommi Jaakkola, and Ali Mohammad. 6.867 Machine Learning. Fall 2006. Massachusetts Institute of Technology: MIT OpenCourseWare, https://ocw.mit.edu. License: Creative Commons BY-NC-SA.

\bibitem{22}
Xiang, Shiming, Feiping Nie, and Changshui Zhang. "Semi-supervised classification via local spline regression." IEEE Transactions on Pattern Analysis and Machine Intelligence 32.11 (2010): 2039-2053.
\bibitem{23}

Hou, Chenping, et al. "Efficient image classification via multiple rank regression." IEEE Transactions on Image Processing 22.1 (2013): 340-352.

\bibitem{24}
Ng, A. "Lecture notes. CS 229: Machine learning." (2003).

\bibitem{25}
Menzies, T., Krishna, R., Pryor, D. (2016). The Promise Repository of Empirical Software Engineering Data; http://openscience.us/repo. North Carolina State University, Department of Computer Science 

\bibitem{26}
Hall, Mark A. Correlation-based feature selection for machine learning. Diss. The University of Waikato, 1999.

\bibitem{27}
Yu, Lei, and Huan Liu. "Efficient feature selection via analysis of relevance and redundancy." Journal of machine learning research 5.Oct (2004): 1205-1224.

\bibitem{28}
S. Lessmann, B. Baesens, C. Mues, and S. Pietsch. Benchmarking Classification Models for Software Defect Prediction : A Proposed Framework and Novel
Findings. Transactions on Software Engineering, 34(4):485–496, 2008.


\bibitem{29}
Altmann, André, et al. "Permutation importance: a corrected feature importance measure." Bioinformatics 26.10 (2010): 1340-1347.

\bibitem{30}
Strobl, Carolin, et al. "Conditional variable importance for random forests." BMC bioinformatics 9.1 (2008): 1.

\bibitem{31}
Kohavi, Ron. "A study of cross-validation and bootstrap for accuracy estimation and model selection." Ijcai. Vol. 14. No. 2. 1995.

\bibitem{32}
Krstajic, Damjan, et al. "Cross-validation pitfalls when selecting and assessing regression and classification models." Journal of cheminformatics 6.1 (2014): 1.

\bibitem{33}
Witten, Ian H., and Eibe Frank. Data Mining: Practical machine learning tools and techniques. Morgan Kaufmann, 2005.

\bibitem{34}
C. Tantithamthavorn, S. McIntosh, A. E. Hassan, and K. Matsumoto. Comments on “Researcher Bias: the Use of Machine Learning in Software Defect Prediction”. PeerJ PrePrints, page 3:e1543, 2015

\bibitem{35}
Q. Song, Z. Jia, M. Shepperd, S. Ying, and J. Liu. A General Software Defect-Proneness Prediction Framework. Transactions on Software Engineering, 37(3):356–370, 2011.

\bibitem{36}
B. Ghotra, S. McIntosh, and A. E. Hassan. Revisiting the Impact of Classification Techniques on the Performance of Defect Prediction Models. In Proceedings of the International Conference on Software Engineering, pages 789–800, 2015.

\bibitem{37}
Tantithamthavorn, Chakkrit, et al. "Automated parameter optimization of classification techniques for defect prediction models." Proceedings of the 38th International Conference on Software Engineering. ACM, 2016.

\bibitem{38}
T. Mende. Replication of Defect Prediction Studies: Problems, Pitfalls and Recommendations. In Proceedings of the International Conference on Predictive Models in Software Engineering, pages 1–10, 2010.

\bibitem{39}
P. Peduzzi, J. Concato, E. Kemper, T. R. Holford, and A. R. Feinstein. A Simulation Study of the Number of Events per Variable in Logistic Regression Analysis. Journal of Clinical Epidemiology, 49(12):1373–1379, 1996.

\bibitem{40}
Tantithamthavorn, Chakkrit, et al. "An empirical comparison of model validation techniques for defect prediction models." IEEE Transactions on Software Engineering (2015).

\bibitem{41}
Sarle, W. S. "The VARCLUS procedure." SAS/STAT User's Guide, (1990).

\bibitem{42}
F. Rahman and P. Devanbu. How, and why, process metrics are better. In Proceedings of the International Conference on Software Engineering, pages 432–441, 2013.

\bibitem{43}
H. He and E. A. Garcia. Learning from Imbalanced Data. Transactions on Knowledge and Data Engineering, 21(9):1263–1284, 2009.

\bibitem{44}

Harter, Donald E., Mayuram S. Krishnan, and Sandra A. Slaughter. "Effects of process maturity on quality, cycle time, and effort in software product development." Management Science 46.4 (2000): 451-466.

\bibitem{45}
Boehm, Barry, Hans Dieter Rombach, and Marvin V. Zelkowitz, eds. Foundations of empirical software engineering: the legacy of Victor R. Basili. Springer Science and Business Media, 2005.

\bibitem{46}
Wilcoxon, Frank. "Individual comparisons by ranking methods." Biometrics bulletin 1.6 (1945): 80-83.

\bibitem{47}
 J. Cohen. Statistical Power Analysis for the Behavioral Sciences. 1988.
\bibitem{48}
J. Cohen. A power primer. Psychological bulletin,112(1):155, 1992

\bibitem{49}
C. Tantithamthavorn. Towards a Better Understanding of the Impact of Experimental Components on Defect Prediction Modelling. In Proceedings of the International Conference on Software Engineering, page To appear, 2016.

\bibitem{50}
C. Tantithamthavorn, S. McIntosh, A. E. Hassan, A. Ihara, and K. Matsumoto. The Impact of Mislabelling on the Performance and Interpretation of Defect Prediction Models. In Proceedings of the International Conference on Software Engineering, pages 812–
823, 2015.

\bibitem{51}
Zimmermann, Thomas, Rahul Premraj, and Andreas Zeller. "Predicting defects for eclipse." Predictor Models in Software Engineering, 2007. PROMISE'07: ICSE Workshops 2007. International Workshop on. IEEE, 2007.

\bibitem{52}
Zimmermann, Thomas, and Nachiappan Nagappan. "Predicting defects using network analysis on dependency graphs." Proceedings of the 30th international conference on Software engineering. ACM, 2008.
\bibitem{53}
Zimmermann, Thomas, et al. "Cross-project defect prediction: a large scale experiment on data vs. domain vs. process." Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering. ACM, 2009.

\bibitem{54}
Nagappan, Nachiappan, Thomas Ball, and Andreas Zeller. "Mining metrics to predict component failures." Proceedings of the 28th international conference on Software engineering. ACM, 2006.

\bibitem{55}
Graves, Todd L., et al. "Predicting fault incidence using software change history." IEEE Transactions on software engineering 26.7 (2000): 653-661.

\bibitem{56}
Ying, Annie TT, et al. "Predicting source code changes by mining change history." IEEE Transactions on Software Engineering 30.9 (2004): 574-586.

\bibitem{57}
Hassan, Ahmed E. "Predicting faults using the complexity of code changes." Proceedings of the 31st International Conference on Software Engineering. IEEE Computer Society, 2009.
\bibitem{58}

Guo, Lan, et al. "Robust prediction of fault-proneness by random forests." Software Reliability Engineering, 2004. ISSRE 2004. 15th International Symposium on. IEEE, 2004.

\bibitem{59}
Elish, Karim O., and Mahmoud O. Elish. "Predicting defect-prone software modules using support vector machines." Journal of Systems and Software 81.5 (2008): 649-660.

\bibitem{60}
B. Efron. Estimating the error rate of a prediction rule: improvement on cross-validation. Journal of the American Statistical Association, 78(382):316–331, 1983


\end{thebibliography}


==> Results.tex <==
\subsection{RQ1}
\input{RQ1}


==> ieee_conf/ieee_conf/IEEECS_confs_LaTeX/README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************

